Gradient Inversion of Federated Diffusion Models

Diffusion models are becoming defector generative models, which generate exceptionally high-resolution image data. Training effective diffusion models require massive real data, which is privately owned by distributed parties. Each data party can collaboratively train diffusion models in a federated learning manner by sharing gradients instead of the raw data. In this paper, we study the privacy leakage risk of gradient inversion attacks. First, we design a two-phase fusion optimization, GIDM, to leverage the well-trained generative model itself as prior knowledge to constrain the inversion search (latent) space, followed by pixel-wise fine-tuning. GIDM is shown to be able to reconstruct images almost identical to the original ones. Considering a more privacy-preserving training scenario, we then argue that locally initialized private training noise $\epsilon$ and sampling step t may raise additional challenges for the inversion attack. To solve this, we propose a triple-optimization GIDM+ that coordinates the optimization of the unknown data, $\epsilon$ and $t$. Our extensive evaluation results demonstrate the vulnerability of sharing gradient for data protection of diffusion models, even high-resolution images can be reconstructed with high quality.

==> sections/limitation.tex <==
% \section{Limitations}
% \label{sec:limitation}
% Our experimental results reveal the significance of knowing the Gaussian noise $\boldsymbol{\epsilon}$ for gradient inversion attacks on DDPM. \algp proposes to apply triple optimization and is able to recover the image of size $32 \times 32$ but does fail on larger images. We leave the design of this stronger attack for future work. 
